Pushing the Boundaries of Private, Large-Scale Query Answering

We address the problem of efficiently and effectively answering large numbers of queries on a sensitive dataset while ensuring differential privacy (DP). We separately analyze this problem in two distinct settings, grounding our work in a state-of-the-art DP mechanism for large-scale query answering: the Relaxed Adaptive Projection (RAP) mechanism. The first setting is a classic setting in DP literature where all queries are known to the mechanism in advance. Within this setting, we identify challenges in the RAP mechanism's original analysis, then overcome them with an enhanced implementation and analysis. We then extend the capabilities of the RAP mechanism to be able to answer a more general and powerful class of queries (r-of-k thresholds) than previously considered. Empirically evaluating this class, we find that the mechanism is able to answer orders of magnitude larger sets of queries than prior works, and does so quickly and with high utility. We then define a second setting motivated by real-world considerations and whose definition is inspired by work in the field of machine learning. In this new setting, a mechanism is only given partial knowledge of queries that will be posed in the future, and it is expected to answer these future-posed queries with high utility. We formally define this setting and how to measure a mechanism's utility within it. We then comprehensively empirically evaluate the RAP mechanism's utility within this new setting. From this evaluation, we find that even with weak partial knowledge of the future queries that will be posed, the mechanism is able to efficiently and effectively answer arbitrary queries posed in the future. Taken together, the results from these two settings advance the state of the art on differentially private large-scale query answering.

==> overview.tex <==
\section{Overview of the Approach} \label{sec:overview}
In this section, we provide high level descriptions of and motivations for the approaches that we will take to accomplish our proposed contributions (Section \ref{sec:prop-contributions}).

\subsection{Expanding the Class of Queries}
We now describe the expanded class of queries that we are proposing to evaluate: $r$-of-$k$ thresholds.
We begin with a discussion of the query classes that have been studied in prior works in order to understand their connection to $r$-of-$k$ thresholds as well as to motivate the need for expanding the class of queries.

Prior work on answering statistical queries in practical settings has been focused on relatively simple classes of statistical queries -- most popularly $k$-way marginals, as these are an important and useful query class which is evaluable within a reasonable computational budget~\cite{barak2007privacy, thaler2012faster, gupta2013privately, chandrasekaran2014faster}.
With the introduction of Aydore et al.'s gradient-based Relaxed Projection (\rp) mechanism~\cite{aydore2021differentially}, they claim that \rp\ is able to answer queries from richer classes under two conditions: (1) that EEDQs can be derived which correspond to the original queries, and (2) that answers to those EEDQs can be efficiently computed.
They demonstrated this claim by evaluating a new class of queries, 1-of-$k$ thresholds, in addition to the standard $k$-way marginals.

Although their evaluation attained high utility results on both query classes, the choice to extend from $k$-way marginals to 1-of-$k$ thresholds enabled them to reuse virtually the same class of surrogate queries, and correspondingly, virtually the same highly-optimized NumPy~\cite{numpy} method (\einsum) within JAX~\cite{bradbury2020jax} to efficiently evaluate them.
Thus, the evaluation was not fully convincing in demonstrating that \rp\ is truly effective for richer classes of queries.

Our contribution will be to develop the mathematical and computational machinery necessary to demonstrate the effectiveness of \rp\ on a class of queries which generalizes both $k$-way marginals as well as 1-of-$k$ threshold queries: $r$-of-$k$ threshold queries.
$r$-of-$k$ thresholds have previously received some theoretical attention from the DP community \cite{thaler2012faster, neel2019use}, although no practical evaluations have been done, likely due to the computational difficulty.
Aydore et al.'s mechanism may be able to overcome this difficulty, but requires differentiable surrogate queries for the class of $r$-of-$k$ queries.
However, since $r$-of-$k$ thresholds strictly generalize both $k$-way marginals and 1-of-$k$ thresholds, their previous class of surrogate queries aren't able to trivially represent $r$-of-$k$ thresholds.
Therefore, we must analogously generalize the class of surrogate queries.
Moreover, Aydore et al. relied on clever use of the highly-optimized \einsum\ method to efficiently evaluate their surrogate queries.
We instead seek more straightforward, approachable methods to evaluate our generalized surrogate queries, relying on modern powerful language primitives (such as vectorization, just-in-time-compilation, and static graph optimization) to enable their efficient evaluation.
Once implemented, we will experimentally evaluate the mechanism's utility using the ADULT \cite{frank2010uci} and ACS \cite{ruggles2020ipums} datasets to determine whether or not this approach is effective on the richer class of queries.


\subsection{Extending the Utility Analysis}
We now turn our attention to why and how we intend to extend the utility analysis of the \rp\ mechanism.

In statistical modeling, and especially in the subfield of synthetic data generation, the primary goal isn't to generate a model or synthetic dataset that answers a prespecified set of queries well. 
Rather, the goal is to generate a model or dataset that \textit{generalizes} well to future queries.
When it comes to differentially private mechanisms for answering statistical queries through a synthetic dataset, prior utility analyses have only focused on either: (a) how well those mechanisms answer the prespecified set of queries, or (b) on theoretically bounding how well the mechanisms can answer any set of queries in the worst-case.

However, in practical settings, it may be more useful to analyze how well the mechanism can answer future queries which are similar to the prespecified ones; i.e., analyzing how well the mechanism generalizes.
Concretely, assuming the prespecified queries come from some query distribution, we are interested in how well the mechanism (whose synthetic data was learned using those prespecified queries) is able answer future queries coming from the same distribution.
For \textit{a priori} unknown distributions, this is a challenging problem to approach theoretically without resorting to worst-case guarantees.
Experimentally, however, we intend to efficiently approach this as follows: (1) construct query distributions according to real-world phenomena, (2) sample separate sets of prespecified and ``future'' queries from the same constructed distribution, and then (3) use the ADULT and ACS datasets to empirically evaluate how well the 
mechanism generalizes from the prespecified queries to the future queries.
This is analogous to standard practice in empirical machine learning research where data is split into ``training'' and ``test'' sets randomly (to ensure distributional similarity); the model is then learned on the training set, and subsequently evaluated on the test set to measure how well it generalizes.


\subsection{Incorporating Historical Queries}
For this final component, we describe our proposed method for incorporating information from the past (via historical queries) by combining the expanded class of queries and extended utility analysis.
We describe its motivation, detail some straightforward methods that are unsatisfactory, then provide intuition for why we expect that our proposed method will attain high utility.

Returning to the 2020 US Census example from Section~\ref{sec:prop-summary}, in addition to the queries posed by the US Census Bureau to release their requisite statistics, researchers have also posed many queries of their own on prior census data.
A method which allows the researchers' historically-posed queries to be incorporated into the synthetic data generation process alongside the Census Bureau's prespecified queries has the potential to ensure that if similar queries are posed in the future on the new Census data, then the corresponding answers would retain high utility.

One straightforward approach to answering both the Census Bureau's and the researchers' queries would be to simply combine the prespecified queries directly with the historical queries.
This approach has the advantage of simplicity, but it has some drawbacks.
Primarily, it implicitly assumes that the prespecified and historical queries are of the same importance.
Often in practice, it's the prespecified queries that need to be answered most accurately, and the ability to answer some future queries accurately is essentially a side benefit.
For example, the Census Bureau is mandated release specific prespecified statistics to a certain degree of accuracy; once this is ensured, it's a bonus if researchers' future queries can be answered accurately.
However, there may be other scenarios where the analyst only needs a few rough answers to their queries, and intends to release the synthetic dataset with the hopes that it will be highly accurate for others' future queries.

Another straightforward approach which could remedy previous approach's drawback would be to learn a separate synthetic dataset for each of these two tasks: one synthetic dataset for answering the prespecified queries, and one synthetic dataset (learned on the historical queries) for answering future queries.
With a fixed computational budget and privacy budget, this approach necessitates splitting the size of the synthetic dataset between each group as well as splitting the privacy budget between each group's queries (where the curator specifies the splits as a hyperparameter, based on the relative importance between the two groups of queries).

However, results from the field of multi-task learning~\cite{zhang2021survey} have consistently shown that shared information from multiple related tasks can be leveraged to improve the performance of all the tasks.
Thus, we hypothesize that learning a single joint synthetic dataset for both prespecified queries and future queries will yield higher utility results than either of the straightforward approaches.
The challenge here is in balancing the utility of prespecified queries with the utility of future queries.
In machine learning, when one wants to constrain the optimization or optimize more than one objective simultaneously, it is standard to incorporate the constraints and objectives into the loss function and let the optimization procedure implicitly sort it out.
We can address our challenge by having our loss function be a weighted combination of the loss on the prespecified and historical queries (with some prespecified weight hyperparameter).
Such a hyperparameter would act as a knob that controls the importance of the prespecified queries vs the historical queries.
We will experimentally investigate the effectiveness of this approach on $r$-of-$k$ queries using the ADULT and ACS datasets, comparing against the two aforementioned straightfoward approaches as baselines.

